$\mu_p$- and $\alpha_p$-actions on K3 surfaces in characteristic $p$

We consider $\mu_p$- and $\alpha_p$-actions on RDP K3 surfaces (K3 surfaces with rational double point singularities allowed) in characteristic $p > 0$. We study possible characteristics, quotient surfaces, and quotient singularities. It turns out that these properties of $\mu_p$- and $\alpha_p$-actions are analogous to those of $\mathbb{Z}/l\mathbb{Z}$-actions (for primes $l \neq p$) and $\mathbb{Z}/p\mathbb{Z}$-quotients respectively. We also show that conversely an RDP K3 surface with a certain configuration of singularities admits a $\mu_p$- or $\alpha_p$- or $\mathbb{Z}/p\mathbb{Z}$-covering by a "K3-like" surface, which is often an RDP K3 surface but not always, as in the case of the canonical coverings of Enriques surfaces in characteristic $2$.

==> preamble.tex <==
%Requires:
%\usepackage{amsmath,amssymb,amsthm,mathrsfs}
\RequirePackage{amsmath,amssymb,amsthm,mathrsfs,comment,url,mathtools,enumerate,booktabs,hyperref}

\newcommand{\gmail}{\url{matsumoto.yuya.m@gmail.com}}
\newcommand{\ymweb}{\url{http://yuyamatsumoto.com/}}
\newcommand{\tusmail}{\url{matsumoto_yuya@ma.noda.tus.ac.jp}}
\newcommand{\tusaddress}{Department of Mathematics, Faculty of Science and Technology, Tokyo University of Science}
\newcommand{\tusaddressfull}{Department of Mathematics, Faculty of Science and Technology, Tokyo University of Science, 2641 Yamazaki, Noda, Chiba, 278-8510, Japan}
\newcommand{\tusaddressja}{〒278-8510 千葉県野田市山崎2641 東京理科大学理工学部数学科}
\newcommand{\numail}{matsumoto.yuya@math.nagoya-u.ac.jp}
\newcommand{\nuweb}{http://www.math.nagoya-u.ac.jp/{\textasciitilde}matsumoto.yuya/}
\newcommand{\nuaddress}{Graduate School of Mathematics, Nagoya University}
\newcommand{\nuaddressfull}{Graduate School of Mathematics, Nagoya University, Furocho, Chikusaku, Nagoya, 464-8602, Japan}
\newcommand{\nuaddressja}{名古屋大学大学院多元数理科学研究科}
%\newcommand{\utmsmail}{ymatsu@ms.u-tokyo.ac.jp}
%\newcommand{\utmsweb}{http://www.ms.u-tokyo.ac.jp/{\textasciitilde}ymatsu/}
%\newcommand{\utmsaddress}{Graduate school of mathematical sciences, University of Tokyo}
%\newcommand{\utmsaddressfull}{Graduate School of Mathematical Sciences, University of Tokyo, 3-8-1 Komaba Meguro-ku Tokyo 153-8914, Japan}
%\newcommand{\utmsaddressja}{東京大学大学院数理科学研究科}

\makeatletter
\newcommand{\dateyyyymmdd}{\the\year/\two@digits\month/\two@digits\day} 
\newcommand{\dateyyyymmddja}{\the\year 年\two@digits\month 月\two@digits\day 日} 
\newcommand{\mydate}{\dateyyyymmdd}
\newcommand{\mydateja}{\dateyyyymmddja}
%\date{\mydate}
\makeatother

\renewcommand{\labelenumi}{\textup{(\theenumi)}}
\renewcommand{\labelenumii}{\textup{(\theenumii)}}

\newcommand{\arxivurl}[1]{\url{http://arxiv.org/abs/#1}}
\newcommand{\hidden}[1]{}

\newcommand{\maru}[1]{\raisebox{.12ex}{{\ooalign{\hfil\footnotesize #1\/\hfil\crcr
       \raise.05ex\hbox{\mathhexbox20D}}}}}

\newcommand{\cO}{\mathcal O}
\newcommand{\cL}{\mathcal L}
\newcommand{\cD}{\mathcal D}
\newcommand{\cC}{\mathcal C}
\newcommand{\cZ}{\mathcal Z}
\newcommand{\cW}{\mathcal W}
\newcommand{\cB}{\mathcal B}
\newcommand{\cX}{\mathcal X}
\newcommand{\cY}{\mathcal Y}
\newcommand{\cA}{\mathcal A}
\newcommand{\cR}{\mathcal R}
\newcommand{\cP}{\mathcal P}
\newcommand{\cQ}{\mathcal Q}
\newcommand{\cE}{\mathcal E}
\newcommand{\cU}{\mathcal U}
\newcommand{\cT}{\mathcal T}
\newcommand{\cV}{\mathcal V}
\newcommand{\cS}{\mathcal S}
\newcommand{\cM}{\mathcal M}
\newcommand{\cF}{\mathcal F}
\newcommand{\cI}{\mathcal I}
\newcommand{\cH}{\mathcal H}
\newcommand{\cN}{\mathcal N}
\newcommand{\cG}{\mathcal G}
\newcommand{\cJ}{\mathcal J}
\newcommand{\cK}{\mathcal K}

\newcommand{\bA}{\mathbb A}
\newcommand{\bP}{\mathbb P}
\newcommand{\bZ}{\mathbb Z}
\newcommand{\bQ}{\mathbb Q}
\newcommand{\bC}{\mathbb C}
\newcommand{\bG}{\mathbb G}
\newcommand{\bF}{\mathbb F}
\newcommand{\bN}{\mathbb N}
\newcommand{\bK}{\mathbb K}
\newcommand{\bS}{\mathbb S}
\newcommand{\bR}{\mathbb R}
\newcommand{\bL}{\mathbb L}
\newcommand{\bV}{\mathbb V}
\newcommand{\bH}{\mathbb H}

\newcommand{\fS}{\mathfrak S}
\newcommand{\fm}{\mathfrak m}
\newcommand{\fn}{\mathfrak n}
\newcommand{\fp}{\mathfrak p}
\newcommand{\fq}{\mathfrak q}
\newcommand{\fA}{\mathfrak A}
\newcommand{\fl}{\mathfrak l}
\newcommand{\fC}{\mathfrak C}
\newcommand{\fg}{\mathfrak g}
\newcommand{\fh}{\mathfrak h}

\newcommand{\sC}{\mathscr C}
\newcommand{\sS}{\mathscr S}
\newcommand{\sX}{\mathscr X}
\newcommand{\sI}{\mathscr I}
\newcommand{\sB}{\mathscr B}
\newcommand{\sP}{\mathscr P}
\newcommand{\sY}{\mathscr Y}
\newcommand{\sM}{\mathscr M}
\newcommand{\sR}{\mathscr R}
\newcommand{\sJ}{\mathscr J}
\newcommand{\sL}{\mathscr L}
\newcommand{\sH}{\mathscr H}

\newcommand{\ideall}{\mathfrak{l}}
\newcommand{\idealm}{\mathfrak{m}}
\newcommand{\idealn}{\mathfrak{n}}
\newcommand{\idealp}{\mathfrak{p}}
\newcommand{\idealq}{\mathfrak{q}}
\newcommand{\Lieg}{\mathfrak{g}}
\newcommand{\Lieh}{\mathfrak{h}}
\newcommand{\Liemup}{\mathfrak{m}_p}
\newcommand{\Liealphap}{\mathfrak{a}_p}

\newcommand{\Cartierdual}{{}^{\mathrm{D}}}

\DeclareMathOperator{\Bl}{Bl}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\Specm}{Specm}
\DeclareMathOperator{\Proj}{Proj}
\DeclareMathOperator{\charac}{char}
\DeclareMathOperator{\Pic}{Pic}
\DeclareMathOperator{\Div}{Div}
\DeclareMathOperator{\Cl}{Cl}
\DeclareMathOperator{\ord}{ord}
\DeclareMathOperator{\lcm}{lcm}
\DeclareMathOperator{\Gal}{Gal}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Rep}{Rep}
\DeclareMathOperator{\Frac}{Frac}
\DeclareMathOperator{\ch}{ch}
\DeclareMathOperator{\CH}{CH}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Coker}{Coker}
%\DeclareMathOperator{\ker}{ker}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\Image}{Im}
\DeclareMathOperator{\Coim}{Coim}
\DeclareMathOperator{\NS}{NS}
\DeclareMathOperator{\pr}{pr}
\DeclareMathOperator{\divisor}{div}
\DeclareMathOperator{\Supp}{Supp}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\Gr}{Gr}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Res}{Res}
\DeclareMathOperator{\SO}{SO}
\DeclareMathOperator{\U}{U}
\DeclareMathOperator{\Sh}{Sh}
\DeclareMathOperator{\disc}{disc}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\GSpin}{GSpin}
\DeclareMathOperator{\GSp}{GSp}
\DeclareMathOperator{\HS}{HS}
\DeclareMathOperator{\Hdg}{Hdg}
\DeclareMathOperator{\height}{ht}
\DeclareMathOperator{\splitheight}{sht}
\DeclareMathOperator{\LCM}{lcm}
\DeclareMathOperator{\Isom}{Isom}
\DeclareMathOperator{\Isometry}{Isometry}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\sHom}{\mathcal{H}\mathit{om}}
\DeclareMathOperator{\sExt}{\mathcal{E}\mathit{xt}}
\DeclareMathOperator{\sEnd}{\mathcal{E}\mathit{nd}}
\DeclareMathOperator{\sAut}{\mathcal{A}\mathit{ut}}
%\DeclareMathOperator{\norm}{Nm}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\specialization}{sp}
\DeclareMathOperator{\Spf}{Spf}
\DeclareMathOperator{\ratrank}{ratrank}
\DeclareMathOperator{\trdeg}{trdeg}
\DeclareMathOperator{\mult}{mult}
\DeclareMathOperator{\discrep}{discrep}
\DeclareMathOperator{\totaldiscrep}{totaldiscrep}
\DeclareMathOperator{\Jac}{Jac}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Alb}{Alb}
\DeclareMathOperator{\Fr}{Fr}
\DeclareMathOperator{\Km}{Km}
\DeclareMathOperator{\Spin}{Spin}
\DeclareMathOperator{\Ortho}{O}
\DeclareMathOperator{\Br}{Br}
\DeclareMathOperator{\Trd}{Trd}
\DeclareMathOperator{\spin}{\mathsf{spin}}
\DeclareMathOperator{\gspin}{\mathsf{gspin}}
\DeclareMathOperator{\so}{\mathsf{so}}
\DeclareMathOperator{\Ad}{Ad}
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\Sing}{Sing}
\DeclareMathOperator{\Bir}{Bir}
\DeclareMathOperator{\Fix}{Fix}
\DeclareMathOperator{\spen}{sp}
\DeclareMathOperator{\Autsymp}{Aut_{symp}}
\DeclareMathOperator{\Bij}{Bij}
\DeclareMathOperator{\sign}{sgn}
\let\sgn=\sign
\DeclareMathOperator{\Stab}{Stab}
\DeclareMathOperator{\Dih}{Dih}
\DeclareMathOperator{\Dic}{Dic}
\DeclareMathOperator{\gr}{gr}
\DeclareMathOperator{\SL}{SL}
\DeclareMathOperator{\Di}{Di}
\DeclareMathOperator{\Lie}{Lie}
\DeclareMathOperator{\wt}{wt}
\DeclareMathOperator{\PGL}{PGL}
\DeclareMathOperator{\PSL}{PSL}
\DeclareMathOperator{\gl}{\mathfrak{gl}}
%\DeclareMathOperator{\sl}{\mathfrak{sl}}
\DeclareMathOperator{\Liesl}{\mathfrak{sl}}
\DeclareMathOperator{\pgl}{\mathfrak{pgl}}
\DeclareMathOperator{\Der}{Der}
\DeclareMathOperator{\kod}{kod}
\DeclareMathOperator{\Exc}{Exc}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\Fun}{Fun}
\DeclareMathOperator{\Obj}{Obj}
\newcommand{\dlog}{\mathop{d \log}}
\DeclareMathOperator{\Td}{Td}
\DeclareMathOperator{\td}{td}
\DeclareMathOperator{\Coh}{Coh}
\DeclareMathOperator{\prank}{\mathit{p}-rank}
\DeclareMathOperator{\Ann}{Ann}
\DeclareMathOperator{\Zero}{Zero}
\DeclareMathOperator{\length}{length}
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator{\Frob}{Frob}
\DeclareMathOperator{\Def}{Def}
\DeclareMathOperator{\Ex}{Ex}
\DeclareMathOperator{\DM}{DM}
\DeclareMathOperator{\Tot}{Tot}
\DeclareMathOperator{\Sp}{Sp}
\DeclareMathOperator{\Cart}{Cart}
\DeclareMathOperator{\Map}{Map}
\DeclareMathOperator{\sSpec}{\mathcal{S}\mathit{pec}}
\DeclareMathOperator{\Open}{Open}
\newcommand{\opensof}[1]{\Open({#1})}
\DeclareMathOperator{\Cont}{Cont}
\DeclareMathOperator{\Spa}{Spa}
\DeclareMathOperator{\Fib}{Fib}

\newcommand{\Zar}{\mathrm{Zar}}
\newcommand{\et}{\mathrm{\acute et}}
\newcommand{\crys}{\mathrm{crys}}
\newcommand{\logcrys}{\mathrm{logcrys}}
\newcommand{\st}{\mathrm{st}}
\newcommand{\pst}{\mathrm{pst}}
\newcommand{\hypst}{\textrm{-}\mathrm{pst}}
\newcommand{\dR}{\mathrm{dR}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\cl}{\mathrm{cl}}
\newcommand{\sm}{\mathrm{sm}}
\newcommand{\sep}{\mathrm{sep}}
\newcommand{\Cst}{\ensuremath{C_\st}}
\newcommand{\ur}{\mathrm{ur}}
\newcommand{\abel}{\mathrm{ab}}
\newcommand{\tame}{\mathrm{tame}}
\newcommand{\alg}{\mathrm{alg}}
\newcommand{\textint}{\mathrm{int}}
\newcommand{\red}{\mathrm{red}}
\newcommand{\sing}{\mathrm{sing}}
\newcommand{\sh}{\mathrm{sh}}% strict Henselization
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\pt}{\mathrm{pt}}
\newcommand{\Betti}{\mathrm{B}}
\newcommand{\KS}{\mathrm{KS}}
\newcommand{\nonsm}{\mathrm{nonsm}}
\newcommand{\hens}{\mathrm{h}}
\newcommand{\tors}{\mathrm{tors}}
\newcommand{\perf}{\mathrm{perf}}
\newcommand{\res}{\mathrm{res}}
\newcommand{\Ga}{\mathrm{\bG_a}}
\newcommand{\Gm}{\mathrm{\bG_m}}
\newcommand{\hatGa}{\hat{\bG}_{\mathrm{a}}}
\newcommand{\hatGm}{\hat{\bG}_{\mathrm{m}}}
\newcommand{\hatBr}{\widehat{\Br}}
\newcommand{\hatotimes}{\mathrel{\hat{\otimes}}}
\newcommand{\Pictau}{\Pic^{\tau}}
%\newcommand{\flat}{\mathrm{fl}}
\newcommand{\an}{\mathrm{an}}

%\newcommand{\Tet}{T}
%\newcommand{\Oct}{O}
%\newcommand{\Ico}{I}
\DeclareMathOperator{\Tet}{Tet}
\DeclareMathOperator{\Oct}{Oct}
\DeclareMathOperator{\Ico}{Ico}
\newcommand{\muDih}{\Dih^{\mu}}
\newcommand{\BinDih}{\widetilde \Dih}
\newcommand{\BinTet}{\widetilde \Tet}
\newcommand{\BinOct}{\widetilde \Oct}
\newcommand{\BinIco}{\widetilde \Ico}
\newcommand{\muBinDih}{\widetilde \muDih}

\newcommand{\Het}{H_\et}
\newcommand{\Hetc}{H_{\et,\mathrm{c}}}
\newcommand{\Hcrys}{H_\crys}
\newcommand{\Hlogcrys}{H_\logcrys}
\newcommand{\Dpst}{D_\pst}
\newcommand{\HBetti}{H}
\newcommand{\Hfl}{H_{\mathrm{fl}}}
\newcommand{\Dst}{D_\st}
\newcommand{\HdR}{H_\dR}
\newcommand{\PHet}{PH_\et}
\newcommand{\PHcrys}{PH_\crys}
\newcommand{\PHBetti}{PH}
\newcommand{\etalepi}{\pi^\et}
\newcommand{\proetalepi}{\pi^{\mathrm{pro\et}}}
\newcommand{\piet}{\etalepi}
\newcommand{\toppi}{\pi^{\mathrm{top}}}
\newcommand{\pitop}{\toppi}

%\newcommand{\myhat}{\text{\hspace{-0.1em}\raisebox{-0.9ex}[0.8ex][0.0ex]{\textasciicircum}\hspace{-0.1em}}}


%%\newcommand{\rationalto}{- \to}
%\newcommand{\rationalto}{\to}
%\newcommand{\rationalmapto}{-\to}
\newcommand{\rationalmapto}{\dashrightarrow}
\newcommand{\rationalto}\rationalmapto
\newcommand{\isomto}{\stackrel{\sim}{\to}}
\newcommand{\isomfrom}{\stackrel{\sim}{\leftarrow}}
\newcommand{\injto}{\hookrightarrow}
\newcommand{\isom}{\cong}
\newcommand{\actson}{\curvearrowright}
\newcommand{\from}{\leftarrow}
\newcommand{\surjto}{\twoheadrightarrow}
\newcommand{\surjfrom}{\twoheadleftarrow}
\newcommand{\SSto}{\Longrightarrow}
\newcommand{\functorto}{\Longrightarrow}
\newcommand{\equivalentto}{\Longleftrightarrow}

\newcommand{\divides}{\mid}
%\newcommand{\notdivides}{\!\not\,\mid} %\nmid?
\newcommand{\notdivides}{\nmid} %\nmid?
\newcommand{\dividesexactly}{\mathrel{\divides\divides}}

\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\fracpart}[1]{\{ #1 \}}
\newcommand{\norm}[1]{\lvert #1 \rvert}
\newcommand{\spectralnorm}[2]{\lvert #1 \rvert_{#2,\mathrm{sp}}}
\newcommand{\supnorm}[2]{\lvert #1 \rvert_{\mathrm{sup},#2}}
\newcommand{\tube}[1]{\mathopen]#1\mathclose[}
\newcommand{\spanned}[1]{\langle #1 \rangle}
\newcommand{\spannedHens}[1]{[ #1 ]^\hens}
\newcommand{\polyHens}[1]{[ #1 ]^\hens}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\biggceil}[1]{\biggl\lceil #1 \biggr\rceil}
\newcommand{\biggfloor}[1]{\biggl\lfloor #1 \biggr\rfloor}
\newcommand{\card}[1]{\lvert #1 \rvert}
\newcommand{\restrictedto}[1]{\rvert_{#1}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\cat}[1]{\{#1\}}
\newcommand{\pairing}[2]{\langle #1,#2 \rangle}
\newcommand{\map}[4][\to]{#2 \colon #3 #1 #4}
%\newcommand{\map}[4]{#2 \colon #3 #1 #4}
%\newcommand{\mapto}[3]{\map{\to}{#1}{#2}{#3}}
\newcommand{\namedarrow}[2]{\stackrel{#1}{#2}}
%\newcommand{\namedto}[1]{\namedarrow{#1}{\to}}
\newcommand{\namedto}[1]{\xrightarrow{#1}}
\newcommand{\twoto}{\rightrightarrows}
\newcommand{\twonamedto}[2]{\xrightarrow[#2]{#1}}
\newcommand{\twonamedarrow}[3]{\overset{#1}{\underset{#2}{#3}}}
\newcommand{\twonamedtwoto}[2]{\overset{#1}{\underset{#2}{\rightrightarrows}}}
\newcommand{\namedisomto}[1]{\twonamedto{#1}{\sim}}
\newcommand{\namedfrom}[1]{\xleftarrow{#1}}
\newcommand{\twonamedfrom}[2]{\xleftarrow[#2]{#1}}
\newcommand{\thpower}[2]{{#1}^{(#2)}}
\newcommand{\pthpower}[1]{\thpower{#1}{p}}
\newcommand{\secondpower}[1]{\thpower{#1}{2}}
\newcommand{\positive}[1]{(#1)^{+}}
%\newcommand{\caseof}[1]{\fbox{#1}}
\newcommand{\isolatedfix}[1]{\langle #1 \rangle}
\newcommand{\divisorialfix}[1]{(#1)}
\newcommand{\iffdef}{\namedarrow{\mathrm{def}}{\iff}}
\newcommand{\normalization}[1]{#1^{\mathrm{n}}}
\newcommand{\dual}[1]{#1^{\vee}}
\newcommand{\evenpart}[1]{#1_{\mathrm{ev}}}
\newcommand{\Legendre}[2]{(\frac{#1}{#2})}
\newcommand{\Witt}[2][]{W_{#1}(#2)}
\newcommand{\shortWitt}[2][]{W_{#1}}
\newcommand{\chitop}{\chi_{\mathrm{top}}}
\newcommand{\clopint}[2]{\mathopen[#1,#2\mathclose[}
\newcommand{\symbolicpower}[2]{{#1}^{[#2]}}
\newcommand{\powerbounded}[1]{#1^{\circ}}
\newcommand{\partialdd}[1]{\frac{\partial}{\partial #1}}


\newcommand{\LKIII}{L_{\mathrm{K3}}}
\newcommand{\LK}[1]{L_{\mathrm{K#1}}}
\newcommand{\Bst}{B_\st}
\newcommand{\WO}{W \mathcal{O}}
\newcommand{\WOmega}[1][]{W_{#1} \Omega}

\newcommand{\rI}{\mathrm I}
\newcommand{\rII}{\mathrm {II}}
\newcommand{\rIII}{\mathrm {III}}
\newcommand{\rIV}{\mathrm {IV}}
%\newcommand{\Ell}{\mathrm{Ell}}
%\newcommand{\Ella}{\Ell_{12\mathrm{a}}}
%\newcommand{\Ella}{\Ell_{12}}
\newcommand{\Ella}{E_{12}}

\newcommand{\categoryof}[1]{\cat{\text{#1}}}
\newcommand{\catmod}[1]{\categoryof{$#1$-mod}}
%\newcommand{\catmodules}[1]{\categoryof{$#1$-modules}}
%\newcommand{\catcoherentmodules}[1]{\categoryof{coh.\ $#1$-modules}}
\newcommand{\catcoherentmodules}[1]{(\mathrm{Coh}/#1)}
\newcommand{\opposite}{^{\mathrm{op}}}
%\newcommand{\functorspace}{{\mathord{-}}}
\newcommand{\sheaveson}[1]{\categoryof{Sh/$#1$}}
\newcommand{\presheaveson}[1]{\categoryof{Presh/$#1$}}
%\newcommand{\constantpresheaf}[1]{\underline{#1}^{\mathrm{p}}}
\newcommand{\constantpresheaf}[1]{\prescript{\mathrm{p}}{}{\underline{#1}}}
\newcommand{\constantsheaf}[1]{\underline{#1}}
\newcommand{\presheavesonvar}[1]{\hat{#1}}

\newcommand{\adjointpair}[4]% 3: 1->2, 4: 2->1, (3(1),2)=(1,4(2))
    {\begin{tikzcd}[ampersand replacement=\&]
    #1\arrow[r,shift left=1ex,"#3"name=F]
    \&#2\arrow[l,shift left=1ex,"#4"name=G]
    \arrow[phantom, from=F, to=G, "\dashv" rotate=-90]
\end{tikzcd}}
\newcommand{\adjoints}{\dashv}
\newcommand{\abeliangroups}{\categoryof{Ab}}
\newcommand{\Cov}{\mathsf{Cov}}
\newcommand{\sets}{\mathsf{Sets}}
\newcommand{\finitesets}{\mathsf{FinSets}}
\newcommand{\finiteGsets}{\finitegroupsets{G}}
\newcommand{\finitegroupsets}[1]{#1\text{-}\mathsf{FinSets}}
\newcommand{\groupsets}[1]{#1\text{-}\mathsf{Sets}}
\newcommand{\finiteetale}[1]{\mathsf{FinEt}/#1}
\newcommand{\etalesite}[1]{#1_{\et}}
\newcommand{\etalesheaveson}[1]{\sS(\etalesite{#1})}
\newcommand{\etalepresheaveson}[1]{\sP(\etalesite{#1})}
\newcommand{\closedpoints}[1]{\pointsofdimension0{#1}}
\newcommand{\pointsofcodimension}[2]{\lvert#2\rvert^{#1}}
\newcommand{\pointsofdimension}[2]{\lvert#2\rvert_{#1}}
\newcommand{\underlyingspace}[1]{\lvert#1\rvert}

\makeatletter
\newcommand{\@Extgroup}[3]{\Ext^2_{#1}(#2, #3)}
%\newcommand{\Extgroup}[3]{\Ext^1_{#1}(#2, #3)}%{A}{I}{A},{X}{\cI}{\cO}
\newcommand{\Extgroup}[3]{\@Extgroup{#1}{#3/#2}{#3}}%{A}{I}{A},{X}{\cI}{\cO}
%\newcommand{\Extgroup}[3]{E^1_{#1}(#2, #3)}%{A}{I}{A},{X}{\cI}{\cO}
\newcommand{\WittExtgroup}[4]{\@Extgroup{#1}{#4/#2}{\Witt[#3]{#4}}}%{A}{I}{n}{A},{X}{\cI}{n}{\cO}
%\newcommand{\WittExtgroup}[4]{E^1_{#1}(#2, \Witt[#3]{#4})}%{A}{I}{n}{A},{X}{\cI}{n}{\cO}
\makeatother
\newcommand{\localcohtorsion}[4][2]{\localcoh[#1]{#2}{#3}[#4]}
\newcommand{\localcoh}[3][2]{H^{#1}_{#2}(#3)}


    \DeclareFontFamily{U}{wncy}{}
    \DeclareFontShape{U}{wncy}{m}{n}{<->wncyr10}{}
    \DeclareSymbolFont{mcy}{U}{wncy}{m}{n}
    \DeclareMathSymbol{\Sha}{\mathord}{mcy}{"58} 
\newcommand{\functorspace}{{\mathord{-}}}
\newcommand{\relmiddle}[1]{\mathrel{}\middle#1\mathrel{}}

\newcommand{\TBF}{ ******** \emph{To be filled...} ******** }
%\newcommand{\あとで}{＊＊あとで埋める＊＊}
%\newcommand{\後で}{\あとで}

\newcommand{\emphi}[1]{\textbf{\underline{#1}}}
\newcommand{\emphii}[1]{\underline{#1}}
\newcommand{\subpara}[1]{【\textbf{{#1}}】\quad}

%\newcommand{\bouchu}[1]{\marginpar{********** #1 **********}}
\newcommand{\bouchu}[1]{\marginpar{#1}}



%	\theoremstyle{plain}
%	\newtheorem{thm}{Theorem}[section]
%	\newtheorem{lem}[thm]{Lemma}
%	\newtheorem{prop}[thm]{Proposition}
%	\newtheorem{cor}[thm]{Corollary}
%	\newtheorem{fact}[thm]{Fact}
%	\newtheorem{conj}[thm]{Conjecture}
%	\newtheorem{claim}[thm]{Claim}
%	\newtheorem{defnprop}[thm]{Definition-Proposition}
%	\theoremstyle{definition}
%	\newtheorem{rem}[thm]{Remark}
%	\newtheorem{defn}[thm]{Definition}

\newcommand{\mytheoremstyleenglish}{
 \theoremstyle{plain}
 \newtheorem{thm}{Theorem}[section]
 \newtheorem{lem}[thm]{Lemma}
 \newtheorem{prop}[thm]{Proposition}
 \newtheorem{cor}[thm]{Corollary}
 \newtheorem{fact}[thm]{Fact}
 \newtheorem{claim}[thm]{Claim}
 \newtheorem{assert}[thm]{Assertion}
 \newtheorem*{thm*}{Theorem}
 \newtheorem*{lem*}{Lemma}
 \newtheorem*{prop*}{Proposition}
 \newtheorem*{cor*}{Corollary}
 \newtheorem*{fact*}{Fact}
 \newtheorem*{claim*}{Claim}
 %\newtheorem{defnprop}[thm]{Definition-Proposition}
 \theoremstyle{definition}
 \newtheorem{rem}[thm]{Remark}
 \newtheorem{defn}[thm]{Definition}
 \newtheorem{example}[thm]{Example}
 \newtheorem{conj}[thm]{Conjecture}
 \newtheorem{prob}[thm]{Problem}
 \newtheorem{obs}[thm]{Observation}
 \newtheorem{exer}[thm]{Exercise}
 \newtheorem{step}{Step}
 \newtheorem{setting}[thm]{Setting}
 \newtheorem*{ques}{Question}
 \newtheorem*{rem*}{Remark}
 \newtheorem*{defn*}{Definition}
 \newtheorem*{example*}{Example}
 \newtheorem*{conj*}{Conjecture}
 \newtheorem{conv}[thm]{Convention}
}
\newcommand{\mytheoremstylejapanese}{
 \theoremstyle{definition}
 \newtheorem{thm}{定理}[section]
 \newtheorem{lem}[thm]{補題}
 \newtheorem{prop}[thm]{命題}
 \newtheorem{cor}[thm]{系}
 \newtheorem{fact}[thm]{事実}
 \newtheorem{claim}[thm]{主張}
 %\newtheorem{defnprop}[thm]{Definition-Proposition}
 \newtheorem{rem}[thm]{注}
 \newtheorem{defn}[thm]{定義}
 \newtheorem{example}[thm]{例}
 \newtheorem{conj}[thm]{予想}
 \newtheorem{assum}[thm]{仮定}
 \newtheorem{exer}[thm]{演習問題}
 \newtheorem{prob}[thm]{問題}
 \newtheorem{Cprob}[thm]{チャレンジ問題}
 \newtheorem*{ques}{問題}
 \newtheorem*{thm*}{定理}
 \newtheorem*{cor*}{系}
 \newtheorem*{hope*}{期待}
 \newtheorem*{conj*}{予想}
 \newtheorem*{example*}{例}
 \newtheorem*{defn*}{定義}
 \newtheorem*{rem*}{注}
 \newtheorem{conv}[thm]{語法}
 \newtheorem{deviation}[thm]{余談}
 \renewcommand\proofname{証明.}
}


%%%% カスタマイズ用メモ

%\addtolength{\textheight}{3.5\baselineskip}
%\addtolength{\hoffset}{-30pt}
%\addtolength{\textwidth}{60pt}

%\renewcommand\abstractname{概要}%Abstract
%\renewcommand\contentsname{目次}%Contents
%\renewcommand\refname{参考文献}%References %% or \bibname?
%\renewcommand\datename{更新：}%Date.


%\usepackage[strings]{underscore}%use this to get along with underscores in DOI
